Small Memory Robust Simulation of Client-Server Interactive Protocols over Oblivious Noisy Channels

We revisit the problem of low-memory robust simulation of interactive protocols over noisy channels. Haeupler [FOCS 2014] considered robust simulation of two-party interactive protocols over oblivious, as well as adaptive, noisy channels. Since the simulation does not need to have fixed communication pattern, the achieved communication rates can circumvent the lower bound proved by Kol and Raz [STOC 2013]. However, a drawback of this approach is that each party needs to remember the whole history of the simulated transcript. In a subsequent manuscript, Haeupler and Resch considered low-memory simulation. The idea was to view the original protocol as a computational DAG and only the identities of the nodes are saved (as opposed to the whole transcript history) for backtracking to reduce memory usage. In this paper, we consider low-memory robust simulation of more general client-server interactive protocols, in which a leader communicates with other members/servers, who do not communicate among themselves; this setting can be applied to information-theoretic multi-server Private Information Retrieval (PIR) schemes. We propose an information-theoretic technique that converts any correct PIR protocol that assumes reliable channels, into a protocol which is both correct and private in the presence of a noisy channel while keeping the space complexity to a minimum. Despite the huge attention that PIR protocols have received in the literature, the existing works assume that the parties communicate using noiseless channels.

==> oram.tex <==
\subsection{Application to Multi-Server Perfectly Secure ORAM}


Oblivious RAM (ORAM) protocols~\cite{Goldreich87} allow a client to
outsource storage of its data such that the client can continue
to read/write its data while hiding both the data itself as
well as the client's access pattern. ORAM was historically
considered in the single-server setting, but has recently been
considered in the multi-server
setting~\cite{AbrahamFNP017,GordonKW18,DBLP:conf/tcc/LuO13}
where the client can store
its data on multiple, non-colluding servers. 

Traditionally, the access pattern is obfuscated under the notion of
\emph{computational} security against polynomially bounded adversary,
or \emph{statistical} security against unbounded adversary but with some correctness failure probability.
However, recently \emph{perfect} security against unbounded adversary and with correctness always guaranteed
has been achieved~\cite{DBLP:conf/tcc/DamgardMN11,DBLP:conf/tcc/ChanNS18}.

Nevertheless, ORAM schemes with a single server assumes
that the contents of the underlying blocks are protected using cryptography,
which means eventually these schemes can defend only against polynomially bounded adversaries.


Using random secret sharing, the contents of blocks
can be shared among different servers, thereby eliminating the need
for cryptography.  In addition to removing any cryptographic assumption,
multi-server ORAM also achieves the best known communication overhead
to achieve perfect security, as stated in the following result.



%We address the above questions in this work. (Unless otherwise
%noted, our results hold for arbitrary block size~$B$ as long as
%it is large enough to store an address, i.e., $B = \Omega(\log
%N)$.) We construct a perfectly secure, multi-server ORAM
%scheme that improves upon the overhead of the best known
%construction in the single-server setting. Specifically, we
%show the following --- henceforth
%if a multi-server ORAM scheme
%incurs, on average, $X(N)$ bandwidth (measured in terms of 
%number of blocks transmitted) per logical memory access
%on a logical memory of length $N$, we say that the scheme
%has $X(N)$ {\it bandwidth blowup}. 


\begin{fact}[3-Server Perfectly Secure ORAM~\cite{DBLP:conf/tcc/ChanNS18}]
\label{fact:3-server}
There exists a 3-server ORAM scheme
storing logical $N$ blocks (each of which has size at least $\Omega(\log N)$ bits)
that is perfectly secure against non-colluding servers, 
and achieves on average a communication overhead of $O(\log^2 N)$  blocks per
logical memory access.
Moreover, the client uses $O(1)$ blocks of memory storage,
and each server uses $O(N)$ blocks of memory storage.
%and consumes $O(\log^2
%N)$ bandwidth (measured in terms of number of blocks transmitted)
%per logical memory access on an array of
%length~$N$. 
%Further, our scheme does not rely on server-side
%computation or server-to-server communication. 
\end{fact}

To apply our main Theorem~\ref{th:main}
to the 3-server ORAM in Fact~\ref{fact:3-server},
it suffices that to observe that to serve a sequence of $T$ logical memory accesses
of $W$-bit blocks, the number of bits transmitted in each channel is
$n = T \cdot W \cdot O(\log^2 N)$.
If both $T$ and $W$ are $\poly(N)$, then $\log n = O(\log N)$ and we have
the following result.

\begin{corollary}[3-Server ORAM with Noisy Communication Channel]
Suppose the block size $W$ satisfies $\Omega(\log N) \leq W \leq \poly(N)$,
and the communication channel
between the client and each of the $m =3$ ORAM servers
in Fact~\ref{fact:3-server} has oblivious error rate~$\epsilon$.
Then, using the transformation technique in Theorem~\ref{th:main},
except with probability $\delta = \frac{1}{N^a}$ (where $\omega(1) \leq a \leq \log N$),
the resulting 3-server ORAM achieves security and correctness.
Moreover, 
%the access pattern is statistically secure, and 
the communication overhead is $(1 + O(\sqrt{\epsilon})) \cdot O(\log^2 N)$.

Finally, for a sequence of $T = \poly(N)$ accesses,
the client uses $O(a \log^2 N + W \log N)$ bits of memory,
and each server uses $O(W N \log N)$ bits of storage.
\end{corollary}


%
%
%As a point of comparison, the best known \emph{single-server},
%perfectly secure ORAM schemes require $O(\log^3 N)$
%bandwidth~\cite{oram05,perfectopram}. While
%Theorem~\ref{thm:intromain} holds for any block size
%$B=\Omega(\log N)$, we show that for block sizes $B =
%\Omega(\log^2 N)$
%our scheme achieves bandwidth blowup as small as~$O(\log N)$.



